Incidents1M: a large-scale dataset of images with natural disasters, damage, and incidents

Natural disasters, such as floods, tornadoes, or wildfires, are increasingly pervasive as the Earth undergoes global warming. It is difficult to predict when and where an incident will occur, so timely emergency response is critical to saving the lives of those endangered by destructive events. Fortunately, technology can play a role in these situations. Social media posts can be used as a low-latency data source to understand the progression and aftermath of a disaster, yet parsing this data is tedious without automated methods. Prior work has mostly focused on text-based filtering, yet image and video-based filtering remains largely unexplored. In this work, we present the Incidents1M Dataset, a large-scale multi-label dataset which contains 977,088 images, with 43 incident and 49 place categories. We provide details of the dataset construction, statistics and potential biases; introduce and train a model for incident detection; and perform image-filtering experiments on millions of images on Flickr and Twitter. We also present some applications on incident analysis to encourage and enable future work in computer vision for humanitarian aid. Code, data, and models are available at http://incidentsdataset.csail.mit.edu.

==> old.tex <==
% \begin{table*}[t]
% \FrameSep1pt
% \begin{framed}
% \centering
% \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{lllllll}
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Loss}} & \multicolumn{4}{c}{\textbf{Test set}} \\
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Class-positives}}} & \multicolumn{1}{c}{\textbf{Class-negatives}} & \multicolumn{2}{c}{\textbf{Incidents Dataset \cite{weber2020detecting}}} & \multicolumn{2}{c}{\textbf{Incidents Dataset v2}} \\ \hline
% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Training data}}} &  &  & \multicolumn{1}{c}{Incident mAP} & \multicolumn{1}{c}{Place mAP} & \multicolumn{1}{c}{Incident mAP} & \multicolumn{1}{c}{Place mAP} \\
% Incidents Dataset v2 & \multicolumn{1}{c}{\checkmark} &  & \multicolumn{1}{c}{64.47} & \multicolumn{1}{c}{48.65} & \multicolumn{1}{c}{62.83} & \multicolumn{1}{c}{63.15}  \\
% Incidents Dataset v2 &  \multicolumn{1}{c}{\checkmark} &  \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{66.13} & \multicolumn{1}{c}{49.14} & \multicolumn{1}{c}{67.19} & \multicolumn{1}{c}{62.94}  \\ \hline
% \multicolumn{1}{l}{Incidents Dataset \cite{weber2020detecting}} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{67.72} & \multicolumn{1}{c}{47.58} & \multicolumn{1}{c}{63.89} & \multicolumn{1}{c}{60.33} \\
% \end{tabular}
% \end{framed}
% \caption{\todo{ETHAN: explain this and why the multi-label setting performs best on the multi-label evaluation}}
% \label{table:class_negatives_and_larger_dataset}
% \end{table*}


\begin{table}[t]
\FrameSep1pt
\begin{framed}
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lllllll}
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Loss}} & \multicolumn{4}{c}{\textbf{Test set}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Class-positives}}} & \multicolumn{1}{c}{\textbf{Class-negatives}} & \multicolumn{2}{c}{\textbf{Incidents Dataset v2}} \\ \hline
\multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Training data}}} &  &  & \multicolumn{1}{c}{Incident mAP} & \multicolumn{1}{c}{Place mAP} \\
Incidents Dataset v2 & \multicolumn{1}{c}{\checkmark} &  & \multicolumn{1}{c}{62.83} & \multicolumn{1}{c}{63.15}  \\
Incidents Dataset v2 &  \multicolumn{1}{c}{\checkmark} &  \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{67.19} & \multicolumn{1}{c}{62.94}  \\ \hline
\multicolumn{1}{l}{Incidents Dataset \cite{weber2020detecting}} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{47.58} & \multicolumn{1}{c}{63.89} & \multicolumn{1}{c}{60.33} \\
\end{tabular}
\end{framed}
\caption{\todo{ETHAN: explain this and why the multi-label setting performs best on the multi-label evaluation}}
\label{table:class_negatives_and_larger_dataset}
\end{table}


\subsection{Incidents occurring with people}

Here we aim to understand how often people occur in the Incidents Dataset. Running Mask RCNN provides some insight, be we obtain additional detail by running a pretrained RetinaFace~\cite{deng2019retinaface}
% \footnote{\cite{https://github.com/biubug6/Pytorch_Retinaface}} 
on the images to detect faces and filter with a 0.5 confidence threshold. We report our findings in Fig. \ref{fig:people_analysis}. \dimpp{let's remove this if we don't have something interesting to report or discuss}

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{Assets/PDF/people.pdf}
\caption{Person and face detections. \ethan{todo: describe what this plot shows}}
\label{fig:people_analysis}
\end{figure}

In \cite{luccioni2021using}, a CycleGAN model is used to synthetically a flood an input image, such as a photo of their own home. The goal of this paper is to bring awareness to people about the issue of climate change and the possible futures humanity may face as disasters, such as floods, occur in our home environments. Their model was trained on synthetic data, and here we present similar results but with real data and using StyleGAN2 instead of CycleGAN.


\ethan{Ferda, please write this section}
\ethan{Here we aim to learn if our model exhibits bias based on geographical location of where images are taken. To do this, we use Twitter; we download images associated with geotagged tweets that have natural disaster keywords. From this collection, we separate the tweets into 6 continents. We exclude Antarctica (AN) from our analysis as tweets are not common here. Once separated into continents with tweet GPS metadata, we then obtain ground-truth labels from AMT. To exhaustively evaluate the models, we would have to obtain labels for all 43 incidents, which quickly becomes costly. To speed up analysis, we first group our incident categories into the following 14 super-categories: ``blocked", ``burned-with smoke", ``collapsed-damaged", ``dirty-contaminated", ``drought", ``earthquake", ``flooded", ``fog", ``heavy rainfall", ``landslide", ``on fire", ``snowstorm-snow covered", ``traffic jam", and ``vehicle accident". Next, we sample 1K images from each continent and for each image, we ask 14 binary questions (i.e., Does this image contain X incident?). Finally, we use these labels to obtain a mean average precision (mAP) metric shown in Tab.~\ref{table:geo_model_bias}. We observe that, unsurprisingly, North America has the best mAP. Europe and Africa follow closely behind. As shown in Fig.~\ref{fig:geo_dist}, it is likely that many of our Incidents1M Dataset images are taken in North America and Europe, which could explain bias in our model performance. Further investigation to understand specific failure cases across geography could be of particular importance, especially if a model trained on the Incidents1M Dataset will be deployed in the real world.}
